Incorporating Causal Analysis into Diversified and Logical Response Generation

Although the Conditional Variational AutoEncoder (CVAE) model can generate more diversified responses than the traditional Seq2Seq model, the responses often have low relevance with the input words or are illogical with the question. A causal analysis is carried out to study the reasons behind, and a methodology of searching for the mediators and mitigating the confounding bias in dialogues is provided. Specifically, we propose to predict the mediators to preserve relevant information and auto-regressively incorporate the mediators into generating process. Besides, a dynamic topic graph guided conditional variational autoencoder (TGG-CVAE) model is utilized to complement the semantic space and reduce the confounding bias in responses. Extensive experiments demonstrate that the proposed model is able to generate both relevant and informative responses, and outperforms the state-of-the-art in terms of automatic metrics and human evaluations.

==> sections/derivation.tex <==
In order to make this derivation more general, here we calculate the KL-divergence between two Gaussian distributions which follow $p_{1}(x) \sim \mathcal{N}(\mu_1, \sigma^2_1)$ and $p_{2}(x) \sim\mathcal{N}(\mu_2, \sigma^2_2)$, respectively:

\begin{align*}
&KL(p_{1}(x)||p_{2}(x))=\int p_{1}(x) \log \frac{p_{1}(x)}{p_{2}(x)} d x  \\
&=\int p_{1}(x)\left(\log p_{1}(x) d x-\log p_{2}(x)\right) d x  \\
&=\int p_{1}(x) *\left(\log \frac{1}{\sqrt{2 \pi \sigma_{1}^{2}}} e^{-\frac{\left(x-\mu_{1}\right)^{2}}{2 \sigma_{1}^{2}}}-\log \frac{1}{\sqrt{2 \pi \sigma_{2}^{2}}} e^{-\frac{\left(x-\mu_{2}\right)^{2}}{2 \sigma_{2}^{2}}}\right) d x   \\
&=\int p_{1}(x) *\left(-\frac{1}{2} \log 2 \pi-\log \sigma_{1}-\frac{\left(x-\mu_{1}\right)^{2}}{2 \sigma_{1}^{2}}+\frac{1}{2} \log 2 \pi+\log \sigma_{2}+\frac{\left(x-\mu_{2}\right)^{2}}{2 \sigma_{2}^{2}}\right) d x  \\
&=\int p_{1}(x)\left(\log \frac{\sigma_{2}}{\sigma_{1}}+\left[\frac{\left(x-\mu_{2}\right)^{2}}{2 \sigma_{2}^{2}}-\frac{\left(x-\mu_{1}\right)^{2}}{2 \sigma_{1}^{2}}\right]\right) d x  \\
&=\int\left(\log \frac{\sigma_{2}}{\sigma_{1}}\right) p_{1}(x) d x+\int\left(\frac{\left(x-\mu_{2}\right)^{2}}{2 \sigma_{2}^{2}}\right) p_{1}(x) d x-\int\left(\frac{\left(x-\mu_{1}\right)^{2}}{2 \sigma_{1}^{2}}\right) p_{1}(x) d x  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{1}{2 \sigma_{2}^{2}} \int\left(\left(x-\mu_{2}\right)^{2}\right) p_{1}(x) d x-\frac{1}{2 \sigma_{1}^{2}} \int\left(\left(x-\mu_{1}\right)^{2}\right) p_{1}(x) d x  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{1}{2 \sigma_{2}^{2}} \int\left(\left(x-\mu_{2}\right)^{2}\right) p_{1}(x) d x-\frac{1}{2}  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{1}{2 \sigma_{2}^{2}} \int\left(\left(x-\mu_{1}+\mu_{1}-\mu_{2}\right)^{2}\right) p_{1}(x) d x-\frac{1}{2}  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{1}{2 \sigma_{2}^{2}}\left[\int\left(x-\mu_{1}\right)^{2} p_{1}(x) d x+\int\left(\mu_{1}-\mu_{2}\right)^{2} p_{1}(x) d x+2 \int\left(x-\mu_{1}\right)\left(\mu_{1}-\mu_{2}\right)\right] p_{1}(x) d x-\frac{1}{2}  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{1}{2 \sigma_{2}^{2}}\left[\int\left(x-\mu_{1}\right)^{2} p_{1}(x) d x+\left(\mu_{1}-\mu_{2}\right)^{2}\right]-\frac{1}{2}  \\
&=\log \frac{\sigma_{2}}{\sigma_{1}}+\frac{\sigma_{1}^{2}+\left(\mu_{1}-\mu_{2}\right)^{2}}{2 \sigma_{2}^{2}}-\frac{1}{2}
\end{align*}


==> sections/model_v1.1.tex <==


\subsection{Problem Definition}
\begin{figure*}[!t]
\centering
\includegraphics[scale=0.5]{pictures/figure2_model_overview3.pdf}
\caption{Overview of the proposed SLARM method.}
\label{fig1}
%\vspace{-0.45cm}
\end{figure*}

Our response generation task is defined as, given an input post $\vec{x}= \{x_1,x_2,\cdots, x_{T}\}$ and let the model to generate the corresponding response sequence $\vec{y} = \{y_1,y_2,\cdots, y_{T^{''}}\}$, where $T$ is the length of the post and $T^{''}$ is the length of response.
To address this problem, we propose to generate the response sequence in a sentence-level auto-regressive manner. Firstly, we segment the to-be-generated response into {\it direct responding semantics} and {\it supplementary semantics}:
\begin{equation}
  \vec{y}=\vec{y}_{direct} + \vec{y}_{sup_1} + \vec{y}_{sup_2} + \cdots ,
\end{equation}
where $\vec{y}_{direct}$ represents the {\it direct responding semantics} and $\vec{y}_{sup_n}$ denotes the $n$'th {\it supplementary semantics}.
The {\it direct responding semantics} is generated solely based on the input post utterance:
\begin{equation}
  \vec{y}^{*}_{direct} = argmax\Pr(\vec{y}|\vec{x}),
\end{equation}
while the next {\it supplementary semantics} is produced by auto-regressively take in the previous generated {\it supplementary semantics}, the {\it direct responding semantics} and the input post:
\begin{equation}
  \vec{y}^{*}_{sup_n} = argmax\Pr(\vec{y}|\vec{x},\vec{y}^{*}_{direct},\cdots ,\vec{y}^{*}_{sup_{n-1}}).
\end{equation}
The final output of the model is a concatenation of the generated {\it direct responding semantics} and {\it supplementary semantics}:
\begin{equation}
  \vec{y}^{*}=\vec{y}^{*}_{direct} + \vec{y}^{*}_{sup_1} + \vec{y}^{*}_{sup_2} + \cdots.
\end{equation}


\subsection{Model Overview}
The overview of this proposed method is shown in Figure \ref{fig1} and it contains three major parts:
\begin{itemize}
  \item \textbf{Preprocessing.} The preprocessing part (which is not directly shown in the figure) determines how to create specially-designed training set that is suitable for the proposed sentence-level auto-regressive training scheme. Additionally, this part also includes the necessary preprocessing for building a helpful dialogue topic graph, which is leveraged to guarantee the smooth transition from direct responding semantics to supplementary semantics.
  \item \textbf{Generation of direct responding semantics.} This part takes in the input post and produce a valid direct responding reply, which is implemented by the Seq2seq model. We believe that the direct responding semantics have less diversity and the vanilla Seq2seq model has the ability of modeling such single semantic space.
  \item \textbf{Generation of supplementary semantics.} This part auto-regressively generates supplementary semantics by using a dialogue topic graph enhanced CVAE model. We use CVAE model to expand the semantic space for more diversified response, and leverage the dialogue topic graph to ensure that the diversity does not come at a cost of reducing relevance and coherence. And the dialogue topic graph can also make sure the smooth and natural transition from the direct responding semantics to the supplementary semantics.
\end{itemize}

\subsection{Preprocessing}
\paragraph{Semantic segmentation.}
In order to prepare for the auto-regressive training scheme, we need to preprocess the dataset by firstly segmenting the sentences into direct responding semantics and supplementary semantics. In our experiment, we formulate a hypothesis that the responses can only contain up to one part of supplementary semantics, as more supplementary semantics can cause the conversation topic to deviate from the main track. A simple but effective way of semantically segmenting the responses is used in our preprocessing step, \ie segment according to the punctuation in the sentence. This is because of the fact that the punctuation is often used when the preceding sentences are semantically different from the succeeding sentences. If the to-be-segmented response have no punctuation mark, an [EOS] token is used as the placeholder, representing that this response only contains direct responding semantics. And if the response have multiple punctuation marks, the midmost one is selected as the final cut point. The preprocessing result is shown in Table \ref{tab2}, which is formulated as:
\begin{equation}
  \vec{y}=\vec{y}_{direct} + \vec{y}_{sup} ,
\end{equation}
where
\begin{equation}
  \vec{y}_{direct}=\{y_1,y_2,\cdots, y_{T^{'}}\},
\end{equation}
\begin{equation}
  \vec{y}_{sup}=\{y_{T^{'}+1},y_{T^{'}+2},\cdots, y_{T^{''}}\}.
\end{equation}

 Additionally, when generating supplementary semantics, the model have to take in the input post and the direct responding semantics together. So the [SEP] token \cite{devlin2018bert} is added as the separating symbol between the two sentences, as is depicted in Figure \ref{fig1}.

\begin{table}
\centering
\begin{tabular}{lll}
\toprule
 & Direct semantics & Supplementary semantics\\
\midrule
Resp1:& \textcolor{red}{Yeah, sure!} & [EOS] \\
Resp2:& \textcolor{red}{Yes,} & I had it at McDonald's. \\
Resp3:& \textcolor{red}{Of course!} & It's already ten o'clock p.m.  \\
Resp4:& \textcolor{red}{Nope,} & I've been busy with my work.  \\
Resp5:& \textcolor{red}{Yes, I've had it.} & I tried a new restaurant  that\\
                                           & & features Thai food.\\
\bottomrule
\end{tabular}
\caption{An illustration of the after-preprocessed responses in Table \ref{tab1}. Note that the [EOS] token is used as the indicator when the response doesn't contain any the supplementary semantics.}
\label{tab2}
\end{table}


\paragraph{Dialogue topic graph construction.}
Although generating the {\it direct responding semantics} and the {\it supplementary semantics} separately can produce longer and more informative sentence, it is possible that the two generators produce conflict sentences such as ``I'm hungry now,'' and ``I just now had dinner at McDonald’s''. Therefore, we propose to build a dialogue topic graph to guarantee the smooth and natural transition from the two semantics. The dialogue topic graph is denoted as $\mathcal{G(V,E)}$, where $\mathcal{V}$ is the set of all the dialogue topic words and $\mathcal{E}$ is all the relations between the topics. For the input post, we extract the topic words based on a TF-IDF method and remove all the stop words. These topic words together make the whole node set $\mathcal{V}$. The edge is set up between the post's topic words $v_i$ and the response's topic words $v_j$, and the weight of the edge is calculated by the equation:
\begin{equation}
  \Pr(e_{ij})=\frac{cnt(e_{ij})}{\sum^n_{j=1}cnt(e_{ij})},
\end{equation}
where $cnt(\cdot)$ denotes the number of occurrence and $e_{ij}$ represents the edge between node $v_i$ and $v_j$.


\subsection{Direct Responding Semantics Generator}

Since most of the chit-chat questions should have some doubt that need to be clarified, the direct responding semantics is an essential part of the response that contains straightforward answer to the question, otherwise the response may seem off-the-topic. The {\it direct responding semantics} is more closely related to the input post than the {\it supplementary semantics} and has less diversity.
Therefore, the Seq2seq-model with attention mechanism is utilized as the {\it direct responding semantics} generator (DRSG).

\subsubsection{Seq2seq with Attention Model}

The Seq2seq-attention model first encodes the input sequence  $\vec{x}= \{x_1,x_2,\cdots, x_{T}\}$ into a series of hidden representations $\vec{h} = (\vec{h}_1,\vec{h}_2,\cdots, \vec{h}_{T})$, and the hidden states are summed up into the context vector using the attention weight:
%
\begin{equation}
  \vec{c}_{t}=\sum_{j=1}^{T}\vec{\alpha}(\vec{s}_{t-1},\vec{h_j})\cdot \vec{h_j},
\end{equation}
%
where $\vec{s}_{t-1}$ is the hidden state of the decoder and $\vec{\alpha}(.,.)$ is the attention score estimated by each input token's contribution to predicting the target word $y_t$ . The decoder iteratively update its hidden state $\vec{s}_t$ using previously generated word $\vec{y}_{t-1}$, previous hidden state $\vec{s}_{t-1}$ and the context vector $\vec{c_t}$, namely,
%
\begin{equation}
  \vec{s}_t = f(\vec{s}_{t-1},\vec{y}_{t-1},\vec{c_t}),\quad\quad t  = 1, 2, \cdots, {T^{'}},
\end{equation}
%
where $f(.,.,.)$ is the RNN-based transformation function ~(\eg LSTM~\shortcite{hochreiter1997long} or GRU~\shortcite{chung2014empirical}). Then, the output distribution of generating the $t$-th token $y_t$ conditioned on the input sequence $\vec{x}$ and the previous predicted word sequence $y_{1:t-1}$
is estimated by
%
\begin{equation}
\begin{array}{ll}
\Pr \left( y_t|y_{1:t-1}, \vec{x}\right)
%
=g(\vec{y}_{t-1},\vec{s_t})
,
\end{array}
\end{equation}
%
where $g(.,.,)$ is the softmax function to produce probability distribution over the vocabulary. Given the preprocessed training data $D$, the DRSG is optimized using log likelihood as the objective for maximization:
\begin{equation}
  \mathcal{L} = \sum_{(\vec{x},\vec{y}_{direct})\in D}log\Pr(\vec{y}_{direct}|\vec{x}).
\end{equation}


\subsection{Supplementary Semantics Generator}

\begin{figure*}[!t]
\centering
\includegraphics[scale=0.45]{pictures/figure3_model.pdf}
\caption{Overview of the proposed method.}
\label{fig2}
%\vspace{-0.45cm}
\end{figure*}

The {\it supplementary semantics} is of great importance to provide useful information for the interlocutors, and it can be rendered as an explanation, supplement or extension of the previous  {\it direct responding semantics.} This semantic part has great diversity, and contains many relevant entities. We propose a novel model, \ie topic graph guided CVAE model (TGG-CVAE), to expand the semantic space in the conversation and sample more diversified and relevant sentence, and leverage the dynamic guidance from the dialogue topic graph to provide smooth and natural transition from the {\it direct responding semantics} to the {\it supplementary semantics}. The model structure is depicted in Figure \ref{fig2}. Need to note that, we also consider the possible circumstance where the responses don't contain any {\it supplementary semantics} by leveraging the [EOS] token as the placeholder. If the TGG-CVAE model predicts [EOS] token at the first time step, this indicates that the direct responding semantics is already complete and it don't need and {\it supplementary semantics}.

\subsubsection{Dynamic Topic Graph Guided CVAE Model}

To generate the supplementary semantics of the response, the proposed TGG-CVAE model takes in the input post and previously generated direct semantics response. We denote the input $\vec{\oldhat{x}}$ as:
\begin{equation}
\vec{\oldhat{x}} = \{x_1, x_2, ..., x_T, [SEP], y_1, y_2, ..., y_{T^{'}} \},
\end{equation}
where the [SEP] token is a special token to separate the two sentences \cite{devlin2018bert}. The goal of this model is to generate the {\it supplementary semantics}:
\begin{equation}
  \vec{y}_{sup}=\{y_{T^{'}+1},y_{T^{'}+2},\cdots, y_{T^{''}}\}.
\end{equation}

The dynamic topic graph guided CVAE model consists of four components: the prior network, the posterior network, topic guide network, and the decoding network. The prior network is trained to approximate $p_\theta(z|\hat{x})$ while the posterior network is trained to approximate $q_\psi(z|\hat{x},\vec{y}_{sup})$, where $\theta$ and $\psi$ are the network parameters and $z$ is the latent variable. Here, $z$ is assumed to follow multivariate Gaussian distribution \cite{zhao2017learning} and then we have:
\begin{align}
 p_{\theta}(z|\hat{x}) & \sim \mathcal{N}(\mu, \sigma^2\mathbf{I}) \\
 q_\psi(z|\hat{x},\vec{y}_{sup}) &  \sim \mathcal{N}(\mu^\prime, \sigma^{\prime 2}\mathbf{I})
\end{align}
Typically, the prior network and the posterior network are RNN-based encoders that transforms the input $\vec{\oldhat{x}}$ and $\vec{y}_{sup}$ into hidden states, and the last hidden state is denoted as $\vec{h_x}$ and $\vec{h_y}$ respectively. The latent variable is estimated by parameterizing its mean and log variance:
\begin{align}
    \begin{bmatrix}
        \mu \\
        \log(\sigma^2)
    \end{bmatrix} & = W_p(\vec{h_x}) + b_p  \\
    \begin{bmatrix}
        \mu^\prime \\
        \log(\sigma^{\prime 2})
    \end{bmatrix} & = W_r
    \begin{bmatrix}
        \vec{h_x}\\
        \vec{h_y}
    \end{bmatrix} + b_r
\end{align}
where the $W_p$, $W_r$ and $b_p$, $b_r$ are the weights and biases for the prior network and posterior the  network respectively. Reparametrization trick \cite{kingma2013auto} is used to obtain the samples from the distributions, where we get $\vec{z}$ from the prior network and $\vec{z^{'}}$  from the posterior network.

For vanilla CVAE model, $\vec{z}$ or $\vec{z^{'}}$ is directly fed as the input of the decoder for decoding from the semantic space. However, as aforementioned, the latent semantic space is too large to train well and the sampling step add randomness to the model. Therefore, although the vanilla CVAE model can generate diversified responses, these responses often have low relevance with the input sequence and are not answering the question. Therefore, we propose to exploit the dialogue topic graph to complement the semantic space and provide more relevant information to enhance the diversity and relevance of the response simultaneously.

Firstly, the topic words $w_1, w_2, ..., w_m$ are extracted from $\vec{\oldhat{x}}$ using TF-IDF method, and then they are put in to the dialogue topic graph to find their nearest $n$ neighbours $w_{11}, w_{12}, ..., w_{mn}$ according to the weight, where $w_{ij}$ is the $j$-th neighbour of the topic word $w_{i}$. We then choose the neighbour with the highest probability:
\begin{equation}
  t_0, t_1, ...,t_K = topK(\Pr(e_{w_iw_{ij}})),
\end{equation}
where we again use the edge probability to select top K topic words, namely, $t_0, t_1, ...,t_K$.

Secondly, since the these topic words contribute differently to the generation of response, we leverage the sampled latent variable to formulate a prior/posterior selection of the topic words. The sampled latent variables  $\vec{z}$ (testing) or $\vec{z^{'}}$ (training) are passed through a projection layer to produce a distribution over the K topic words, namely $\vec{\alpha} =\alpha_1,\alpha_2,...,\alpha_K $. The final representation of the topic information is formulated as a weighted summation of the topic embeddings:
\begin{equation}
  \vec{t} = \alpha_i \cdot \vec{t_i}, \quad i=1,2,3,...,k
\end{equation}
where $\vec{t_i}$ is the embedding of the word $t_i$.

Thirdly, the topic information $\vec{t}$ and the sampled latent variable $\vec{z}$ or $\vec{z^{'}}$ is fed into the decoder, for generating the supplementary semantics, which involves an intractable marginalization over the latent variables. Following \cite{sohn2015learning}, we train the proposed model by maximizing the variational lower bound of the conditional log likelihood:
\begin{align}
  \mathcal{L}_{ELBO} =& -KL(q_{\psi}(\vec{z}|\hat{x},\vec{y}_{sup})||p_\theta(\vec{z}|\hat{x})) \notag \\
  & + {\rm E}_{q_{\psi}(\vec{z}|\hat{x},\vec{y}_{sup})}[{\rm log}\, p_\theta(\vec{y}_{sup}|\vec{z},\hat{x},\vec{t})],
\end{align}
where the $KL(.,.)$ denotes the KL-divergence of the two distributions. 

Since the latent semantic distribution is easy to collapse (\aka  KL-collapse problem), we add bow loss $\mathcal{L}_{BOW}$ and use KL-annealing strategy to deal with the this problem \cite{zhao2017learning}. The final loss function is formulated as:
\begin{equation}
  \mathcal{L} = \mathcal{L}_{ELBO} + \mathcal{L}_{BOW}
\end{equation}

